Wide Network Learning with Differential Privacy

Despite intense interest and considerable effort, the current generation of neural networks suffers a significant loss of accuracy under most practically relevant privacy training regimes. One particularly challenging class of neural networks are the wide ones, such as those deployed for NLP typeahead prediction or recommender systems. Observing that these models share something in common--an embedding layer that reduces the dimensionality of the input--we focus on developing a general approach towards training these models that takes advantage of the sparsity of the gradients. More abstractly, we address the problem of differentially private empirical risk minimization (ERM) for models that admit sparse gradients. We demonstrate that for non-convex ERM problems, the loss is logarithmically dependent on the number of parameters, in contrast with polynomial dependence for the general case. Following the same intuition, we propose a novel algorithm for privately training neural networks. Finally, we provide an empirical study of a DP wide neural network on a real-world dataset, which has been rarely explored in the previous work.

==> est-ub-new.tex <==
\section{Improving DP ERM by sparsity}
\label{sec:dp-erm}

In Section~\ref{sec:erm_1}, we provide our theoretical results for $(\eps,\delta)$-DP non-convex ERM problems under the assumption of sparse gradients. In Section~\ref{sec:erm_2}, we show that for a broad class of problems, i.e., generalized linear models, sparse input leads to sparse gradients.
\subsection{Private ERM with sparse gradients}
\label{sec:erm_1}
We consider the following empirical risk minimization problem: given a training data set $D$ consisting of $n$ data points $D = \{d_j\}_{j=1}^{\ns}$, where
$d_j \in \RR^p$, a constraint set $\cW \in \RR^p$,
and a loss function $\ell\colon \cW \times \RR^{\dims} \rightarrow \RR$, we
want to find
$w^\textit{erm} = \arg\min_{w\in \cW} ~L(w;D) = \arg\min_{w\in \cW} ~
\frac1\ns{\sum_{j=1}^{\ns} \ell(w; d_j)}$ satisfying differential privacy. 

% To characterize the gradient sparsity, we assume the data set has the following structure: $D$ can be evenly divided into $m$ subsets, such that the sum of the gradients of each subset is sparse. Specifically, we let $D = \{ D_1, \ldots,D_m\}$, where $D_1= \{d_1,\ldots,d_{\frac{\ns}{m}}\}, D_2= \{d_{\frac{\ns}{m}+1},\ldots,d_{\frac{2\ns}{n}}\}$, \dots, and $D_{m}= \{d_{\frac{(m-1)\ns}{m}+1},\ldots,d_{\ns}\}$, such that
% \begin{align}
% \label{equ:group_sparsity}
% \forall i \in [m],~~ \normz{\sum_{d_j \in D_i} \nabla \ell(w;d_j)} \le c_1,~\text{for all}~ w \in W.
% \end{align}

% Roughly speaking, this assumption requires that the original dataset can be partitioned into several parts, so that each part exhibits some sparsity similarity.

% This assumption may appear overly strict. However, we justify that it can be satisfied in many real applications. For example, in recommender systems, samples collected from the same user usually have overlapping supports, leading to input sparsity \cite{hu2017mitigating}. In these scenarios, it is natural to partition the input dataset according to the user ID. %Similarly, in NLP, training samples are collected from different sources, where each source usually exhibits some similarity. 
% Similarity also exists in NLP, where training samples are collected from different sources.
% In Section~\ref{sec:erm_2}, we show that for a broad class of problems, sparse input always produces sparse gradients.

% We note that the sparsity assumption is used to argue the \emph{utility} guarantee of our algorithm for non-convex ERM problems, without being necessary for its \emph{privacy}.

To characterize the gradient sparsity, we assume the data set has the following structure:
\begin{align}
\label{equ:group_sparsity}
\forall j \in [\ns],~~ \normz{\nabla \ell(w;d_j)} \le c_1,~\text{for all}~ w \in W.
\end{align}
In Section~\ref{sec:erm_2}, we show that for a broad class of problems, sparse input always produces sparse gradients.

To this end we propose Algorithm~\ref{alg:privatelr}. Intuitively, in each iteration the algorithm first selects the most competitive coordinates of the gradient, and then only adds noise to them. Finally it updates the model according to the noisy version of the gradient. We provide the privacy guarantee and theoretical guarantees in Theorems~\ref{thm:ermpri} and~\ref{thm:erm}.


%
%\begin{algorithm}
%    \caption{Differentially private ERM}
%   \label{alg:privatelr}
%    \begin{algorithmic}[1]
%    \STATE {\bfseries Input:}  Data set $D = \{d_j\}_{j=1}^{\ns} $, loss function $L(w;D)$, privacy parameters $(\eps,\delta)$, constraint set $\cW$, learning rate $\eta_t$, iteration times $T$, and gradient $\ell_\infty$-norm bound $\norminf{\nabla_{\ell(w;d)}}\le c_2$
%    \STATE  Initialize $w_0$ from an arbitrary point in $\cW$
%    \FOR{$t=0$ \text{to} $T-1$}
%    \STATE Pick $D_i \sim_u D$ with replacement 
%      \STATE Compute its average gradient $\nabla_t = \frac{m}{\ns}\sum_{d_j \in D_i} \nabla \ell(w;d_j)$
%      \STATE Let $\Delta_t = \textit{NumericSparse}(\nabla_t, \alpha, c_1, \epsilon^{\prime}, \delta^{\prime})$, where $\dist = \frac{40c_2m \Paren{\log \dims + \log (4c_1 \ns)} \sqrt{c_1\log \frac{2}{\delta^\prime} }}{\ns\eps^\prime}$, $\epsilon^{\prime} = \frac{\epsilon\cdot m}{2\sqrt{2T \log \frac{2}{\delta}}}$ and $\delta^{\prime} = \frac{\delta m}{2T}$
%      \STATE  $w^{t+1} = w_t - \eta_t \Delta_t$    
%     \ENDFOR
%\end{algorithmic}
%\end{algorithm}
\todo{to be changed}
\begin{algorithm}[H]

\KwIn{Data set $D = \{d_j\}_{j=1}^{\ns} $, loss function $L(w;D)$, privacy parameters $(\eps,\delta)$, constraint set $\cW$, learning rate $\eta_t$, iteration times $T$, and gradient $\ell_\infty$-norm bound $\norminf{\nabla{\ell(w;d)}}\le c_2$}

Initialize $w_0$ from an arbitrary point in $\cW$

 \For {$t=0$ \textrm{to} $T$}{
 Pick $D_i \sim_u D$ with replacement 
 
Compute its average gradient $\nabla_t = \frac{m}{\ns}\sum_{d_j \in D_i} \nabla \ell(w_t;d_j)$
 
 Let $\Delta_t = \textit{NumericSparse}(\nabla_t, \alpha, c_1, \epsilon^{\prime}, \delta^{\prime})$, where $\dist = \frac{40c_2m \Paren{\log \dims + \log (4c_1 \ns)} \sqrt{c_1 \cdot \frac{n}{m}\log \frac{2}{\delta^\prime} }}{n\eps^\prime}$, $\epsilon^{\prime} = \frac{\epsilon\cdot m}{2\sqrt{2T \log \frac{2}{\delta}}}$ and $\delta^{\prime} = \frac{\delta m}{2T}$ \
 
 $w_{t+1} = w_t - \eta_t \Delta_t$\
 }


\caption{Differentially private ERM with sparse gradients }
\label{alg:privatelr}
\end{algorithm}


\begin{theorem}[Privacy]
\label{thm:ermpri}
With the assumption that $T \ge 10 m^2$, Algorithm~\ref{alg:privatelr} satisfies $(\eps,\delta)$-DP. 
\end{theorem}
\smallskip
%
 \begin{proof}
 We note that in each iteration, when fixing the randomness due to sampling, step 4 itself satisfies $( \epsilon^{\prime}, \delta^{\prime})$-DP, where $\epsilon^{\prime} = \frac{\epsilon\cdot m}{2\sqrt{2T \log \frac{2}{\delta}}}$ and $\delta^{\prime} = \frac{\delta m}{2T}$. Then by the sampling property of differential privacy (Lemma~\ref{lem:dp_sample}), each iteration ensures $(\frac{\epsilon}{\sqrt{2T \log \frac{2}{\delta}}}, \frac{\delta}{2T})$-DP. To conclude the proof, we apply the strong composition theorem (Lemma~\ref{lem:advcomp}) with $\tilde{\delta} = \frac{\delta}{2}$ and $k=T$.
 \end{proof}

\todo{to be changed}
\begin{theorem}[Utility]
\label{thm:erm}
We assume $\forall d,~\ell(w;d)$ is $K$-smooth; $\forall w,d$, $\norminf{\nabla{\ell(w;d)}}\le c_2$ and $\norm{\nabla{\ell(w;d)}}\le G$. Furthermore, under the assumption \eqref{equ:group_sparsity},
\vspace{-8pt}
\begin{enumerate}
\item If $L(w^0;D) - L(w^*;D) \le D_{L}$, and we set $T = \min \Paren {\frac{m^2}{100},\ns}$, then
%then with probability at least $1-\beta$ over the randomness of the algorithm,
\begin{align}
\expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla L (w_t)}^2} = \widetilde{O}\Paren{\frac{G\Paren{c_1c_2+ \sqrt{K D_{\ell } }}} {\eps}  \Paren{\frac1{m}+\frac1{\sqrt{\ns}} }}. \nonumber
\end{align}
%Furthermore, if $\forall d$, $\ell(w;d)$ is convex,
%\begin{align}
%\min \Paren{ L(w_t;D) - L(w^*;D)  } = \widetilde{O}\Paren{ \frac{ c_1 c_2 D_{L} }{\ns \eps}+\frac{ c_1 c_2^{1.5} \sqrt{ D_{\ell } }    } {\sqrt{\ns\eps L}}  }. \nonumber
%\end{align}
\item
Assume that for all $d$,  $\ell(w;d)$ is convex in $w$, and $\forall t$, $\norm{w_t - w^*} \le D_w$. Let $T = \min \Paren {\frac{m^2}{100},\ns}$, then
\begin{align}
\expectation{\frac1T \sum_{t=1}^{T} \Paren{ L(w_t;D) - L(w^*;D) }}=\widetilde{O}\Paren{\frac{D_w\Paren{G+c_1c_2}} {\eps} \cdot \Paren{\frac1{m}+\frac1{\sqrt{\ns}} }}. \nonumber
\end{align}

\end{enumerate}

\end{theorem}

 \begin{proof}

 First by the privacy guarantees of the sparse vector technique (Lemma~\ref{lem:sparsel2}), for each iteration with probability greater than $1-\frac1{n}$,
 \begin{align}
 &\norm{\nabla_t - \Delta_t} \le \frac{100c_1 c_2 \sqrt{T}\Paren{\log \dims + \log(4c_1\ns) } \log \frac{T}{m\delta}}{\ns\eps}, \nonumber
 \end{align}
where we remark that the sensitivity upper bound is $s_\infty = \frac{2c_2m}{\ns}$.

Note that from the assumption $\norm{\nabla_t - \Delta_t} \le 2G$ for sure. Therefore, 
 \begin{align}
 \expectation{\norm{\nabla_t - \Delta_t}} &\le \frac{100c_1 c_2 \sqrt{T}\Paren{\log \dims + \log(4c_1\ns) } \log \frac{T}{m\delta}}{\ns\eps}+\frac{G}{\ns}\nonumber \\
 &\le \frac{200 c_1 c_2 \sqrt{T}\Paren{\log \dims + \log(4c_1\ns) } \log \frac{T}{m\delta}}{\ns\eps}\nonumber.
 \end{align}
 where the second inequality comes from the fact that $T\ge 1$, and the second term dominates.
 
 Now we need the following lemma. The first half comes from~\cite{AgarwalSYKM18}, and we prove the second half of the lemma in Appendix~\ref{app:proof}.
 %\begin{lemma}(Corollary 1 in~\cite{AgarwalSYKM18})
 \begin{lemma}
 \label{lem:theer}
 Suppose $\forall d$, $\ell(w;d)$ is $K$-smooth, with $\norm{\nabla{\ell(w;d)}}\le G$. Let $w^0$ satisfy $L(w^0;D) - L(w^*;D) \le D_{L}$. Let $\eta \coloneqq \min \Paren{ \frac1K, \sqrt{2D_L} \Paren{\sigma \sqrt{KT}}^{-1} }$, then after $T$ rounds,
 $$
 \expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla L (w_t)}^2} \le \frac{2D_{L} K}{T} + \frac{2\sqrt{2} \sigma \sqrt{K D_{L}}} {\sqrt{T}}+ GB.
 $$
Besides, if we further assume $\forall d$, $\ell(w;d)$ is convex, and $\forall t \in [T]$, $\norm{w_t - w^*} \le D_w$. Let $\eta \coloneqq \min \Paren{ \frac1K, D_w \Paren{\sigma \sqrt{T}}^{-1} }$, then after $T$ rounds.
 \begin{align}
 \expectation{\frac1T  \sum_{t=1}^T \Paren{ L(w_t;D) - L(w^*;D) }}  \le \frac{D_w^2 K}{T} + \frac{D_w \sigma}{\sqrt{T}}+ 2B D_w\Paren{1 + \frac{G}{\sigma \sqrt{T}}}, \nonumber
 \end{align}
 where 
 \begin{align}
 &\sigma^2 = 2\max_{1\le t \le T} \expectation{\norm{\nabla_{t} -\nabla L(w_t;D)}^2 } + 2\max_{1\le t \le T} \expectation{\norm{\nabla_{t} - \Delta_t}^2}, \text{and} \nonumber\\ 
 &B^2= 2\max_{1\le t \le T} \expectation{\norm{\nabla_{t} - \Delta_t}^2}. \nonumber
 \end{align}
 \end{lemma}

 %Note that $\ell$ is $(\sqrt{c_1}c_2)$-Lipschitz, since $\norm{\nabla_{\ell(w;d)}} \le \sqrt{c_1}c_2$. 

First we consider the non-convex setting. By the definition of $B$ and $\sigma$ in Lemma~\ref{lem:theer}, we have $B = \frac{300 c_1 c_2 \sqrt{T}\Paren{\log \dims + \log(4c_1\ns) } \log \frac{T}{m\delta}}{\ns\eps}$, and $\sigma^2 = 2B^2 + 2G^2$. Therefore,
 \begin{align}
 \expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla L (w_t)}^2 } &\le \frac{2D_{L} K }{T}+ \frac{4\sqrt{2} (B+G) \sqrt{K D_{\ell }}} {\sqrt{T}} + GB.  \nonumber
 \end{align}
 %We take $T = \min \Paren {\frac{m^2}{100},\ns}$. 
Suppose $m>10\sqrt{\ns}$, where $T=\min\Paren{\frac{m^2}{100},\ns} = n$. By Lemma~\ref{lem:theer}, 
 \begin{align}
 \expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla L (w_t)}^2}  &= O\Paren{ \frac{ D_{L} K }{\ns}+ \frac{ G \sqrt{K D_{\ell }}} {\sqrt{\ns}} +\frac{ c_1 c_2 G  \Paren{\log \dims + \log(4c_1\ns) } \log \frac{m}{\delta}  } {\sqrt{\ns}\eps}  }\nonumber\\
 & = \widetilde{O}\Paren{\frac{G\Paren{c_1c_2+ \sqrt{K D_{\ell } }}    } {\sqrt{\ns}\eps}  }. \nonumber
 \end{align}
We then consider the case when $m\le 10\sqrt{\ns}$, where $T={\frac{m^2}{100}}$. Note that $\frac1{m} \ge \frac{m}{100n}$.
 \begin{align}
 \expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla L (w_t)}^2}  &= O\Paren{ \frac{ D_{L} K }{m^2}+ \frac{ G \sqrt{K D_{\ell }}} {m} +\frac{ c_1 c_2 m G  \Paren{\log \dims + \log(4c_1\ns) } \log \frac{m}{\delta}  } {\ns\eps}  }\nonumber\\
 & = \widetilde{O}\Paren{\frac{G\Paren{c_1c_2+ \sqrt{K D_{\ell } }}    } {m\eps}  }. \nonumber
 \end{align}
 Therefore, 
 \begin{align}
 \expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla L (w_t)}^2} = \widetilde{O}\Paren{\frac{G\Paren{c_1c_2+ \sqrt{K D_{\ell } }}} {m\eps}  }+\widetilde{O}\Paren{\frac{G\Paren{c_1c_2+ \sqrt{K D_{\ell } }}} {\sqrt{\ns}\eps}}, \nonumber
 \end{align}
 and we have proved the first part of Theorem~\ref{thm:erm}.

 Similarly, for convex loss functions,
 \begin{align}
 \expectation{\frac1T  \sum_{t=1}^T\Paren{ L(w_t;D) - L(w^*;D) }  } &\le \frac{D_w^2 K}{T} + \frac{D_w (B+G )}{\sqrt{T}}+ 2B D_w\Paren{1 + \frac{G}{(B+G)\sqrt{T}}}. \nonumber\\
 &\le \frac{D_w^2 K}{T} + \frac{D_w G}{\sqrt{T}}+ 2B D_w. \nonumber
 \end{align}
 If we take $T =\min(\frac{m^2}{100},\ns)$, and by similar arguments,
 % \begin{align}
 % \frac1T  \expectation{\sum_{t=1}^T \Paren{ L(w_t;D) - L(w^*;D) }}  &= O\Paren{  \frac{D_w^2 K \sqrt{c_1}}{\ns\eps} + \frac{D_w c_1^{\frac{3}{4}} c_2 }{\sqrt{\ns\eps}}+ \frac{2D_w c_1^{\frac{3}{4}} c_2  \Paren{\log \dims + \log(4c_1\ns) } \log \frac{T}{\ns\delta}}{\sqrt{\ns\eps}}  } \nonumber\\
 % &= \widetilde{O}\Paren{ \frac{D_w^2 K \sqrt{c_1}}{\ns\eps} + \frac{D_w c_1^{\frac{3}{4}} c_2 }{\sqrt{\ns\eps}}}.\nonumber
 % \end{align}
 \begin{align}
 \expectation{\frac1T \sum_{t=1}^T \Paren{ L(w_t;D) - L(w^*;D) }}  &=  \widetilde{O}\Paren{ \frac{D_w (G+c_1c_2)}{\sqrt{\ns}\eps} + \frac{D_w (G+c_1c_2)}{m\eps}}.\nonumber
 \end{align}

 %For the second part, we need the following property of convex smooth functions:
 %
 %\begin{lemma}
 %\label{lem: property_smooth_convex}
 %Let $\ell$ be a convex and $L$-smooth function on $\mathbb{R}^{\dims}$, 
 %$$f(y) - f(x) - \nabla f (x)^ T (y-x) \ge \frac1{2L} \norm{\nabla f(y) - \nabla f(x)}^2 , ~~~ \forall x,y \in \mathbb{R}^{\dims}.$$\end{lemma}
 %
 %Let $w^{t^\prime} = \arg\min {\ell(w_t;D)}$, by Lemma~\ref{lem: property_smooth_convex},
 %
 %
 %\begin{align}
 %\min \Paren{ L(w_t;D) - L(w^*;D)  } = \widetilde{O}\Paren{ \frac{ c_1 c_2 D_{L} }{\ns \eps}+\frac{ c_1 c_2^{1.5} \sqrt{ D_{\ell } }    } {\sqrt{\ns\eps L}}  }. \nonumber
 %\end{align}

 \end{proof}

\subsection{Sparse features lead to sparse gradients}
\label{sec:erm_2}
In this section, we show that for generalized linear model (GLM), sparse input always leads to sparse gradients. 

%GLM is one of the most fundamental models in statistics and machine learning, which is introduced as a way of unifying various statistical models, including linear, logistic and Poisson regressions. We define GLM as follows:

\smallskip

\noindent\textbf{GLM:}
Let a dataset $D=(x_j, y_j)_{j=1}^\ns$,  where $ \forall j, x_j \in \mathbb{R}^\dims$, and $y_j \in [0, 1]$. Let $\Phi\colon \mathbb{R} \rightarrow \mathbb{R}$ be a \textit{cumulative generating function}. The objective of GLM is to minimize $\frac{1}{n}\sum_{i=1}^n[\Phi(\langle x_i, w\rangle)-y_i\langle x_i, w\rangle]$.

%Let $y\in [0, 1]$ be the response variable that belongs to an exponential family with natural parameter $\eta$. 
% That is, its probability density function can be written as $p(y|\eta)= \exp(\eta y-\Phi(\eta))h(y)$, where $\Phi$ is the \textit{cumulative generating function}. Given observations $y^1, \cdots, y_n$ such that $y_i\sim p(y_i|\eta_i)$ for $\eta=(\eta_1, \cdots, \eta_n)$, the maximum likelihood estimator (MLE) can be written as  $p(y^1,y^2,\cdots|\eta)=\exp(\sum_{i=1}^n y_i\eta_i-\Phi(\eta_i))\Pi_{i=1}^nh(y_i)$. In GLM, we assume that $\eta$ is modeled by linear relations, {\em i.e.,}
%$\eta_i=\langle x_i,  w^*\rangle$ for some $w^*\in \mathbb{R}^p$ and feature vector $x_i$. Thus, maximizing MLE is equivalent to minimizing $\frac{1}{n}\sum_{i=1}^n[\Phi(\langle x_i, w\rangle)-y_i\langle x_i, w\rangle]$.

% The goal is to find $w^*$, which is equivalent to minimizing its population version  
% \begin{equation}\label{eq:1}
%     w^*=\arg\min_{w\in \mathbb{R}^p}\mathbb{E}_{(x,y)}[\Phi(\langle x, w\rangle )- y\langle x, w \rangle ].
% \end{equation}
In the following lemma, we observe that for GLM, sparse input produces sparse gradients. 
\begin{lemma}
For all $x \in \mathbb{R}^\dims$ with $\normz{x}\le c_1$, and $y \in [0,1]$,
$$\normz{\nabla \ell(w;(x,y))} \le c_1.$$
\end{lemma}

\begin{proof}
Note that $\ell(w;(x,y)) = \Phi(\langle x_i, w\rangle)-y_i\langle x_i, w\rangle $, and 
$\nabla \ell(w;(x,y)) = \Paren{\Phi^\prime (\langle x_i, w\rangle)- y_i} \cdot x_i$.  Therefore, $\normz{\nabla \ell(w;(x,y))} \le c_1.$
\end{proof}

As a corollary, for a group of samples $(x_i,y_i)_{i=1}^{\frac{\ns}{m}}$, assuming the non-zero coordinates are the same for each $x_i$ gives the condition in Equation~\eqref{equ:group_sparsity}.
%the average gradient is sparse suppose they share the same set of input features.




==> est-ub_old.tex <==
\section{Private ERM with sparse gradients}

\todo{There is some BUG in the proof, and I will change it. Please DO NOT TOUCH this section until this todo disappears.}
We consider the following empirical risk minimzation problem: given a training data set $D$ consisting of $n$ pairs
of data points $D = \{d^j\}_{j=1}^{\ns}= \{ (x^j, y^j)\}_{j=1}^{\ns}$, where
$x^j \in \RR^p$ and $y^j \in \RR$, a constraint set $\cW \in \RR^p$,
and a loss function $\ell\colon \cW \times \RR^{p+1} \rightarrow \RR$, we
want to find
$w^\textit{erm} = \arg\min_{w\in \cW} ~\cL(w;D) = \arg\min_{w\in \cW} ~
\frac1\ns{\sum_{j=1}^{\ns} \ell(w; d^j)}$ satisfying differential privacy.

To this end we propose the following algorithm:

%\begin{definition}
%A function $\ell : \cC \rightarrow \RR$ is $L_1$-Lipschitz with respect to $\ell_1$ norm, if the following holds.
%$$\forall w_1, w_2 \in \cC, \absv{\ell(w_1) - \ell(w_2)} \le L_1 \norm{w_1-w_2}.$$
%\end{definition}
%
%The performance of the algorithm also depends on the ``curvature" of the loss function, which is defined below, based on the definition of~\cite{Clarkson10, Jaggi13}. 
%A side remark is that this is a strictly weaker constraint than smoothness~\cite{TalwarTZ14}.
%
%
%\begin{definition}[Curvature constant]
%For $\ell:\cC \rightarrow \RR$, $\Gamma_{\ell}$ is defined as 
%$$ \Gamma_{\ell} = \sup_{w_1, w_2 \in \cC, \gamma \in (0,1], w_3 = w_1 + \gamma (w_2-w_1)}\frac{2}{\gamma^2} \Paren{\ell(w_3) - \ell(w_1) - \langle w_3-w_1, \nabla \ell(w_1) \rangle}.$$
%\end{definition}

%In this section, we specifically consider the linear regression problem, where the loss function $\ell(w; d) = \Paren{y - w^T x}^2$.

\begin{algorithm}[H]

\KwIn{Data set $D = \{(x^1,y^1),\cdots,(x^{\ns},y^\ns)\}$, loss function $\cL(w;D)$, privacy parameters $(\eps,\delta)$, constraint set $\cW$, learning rate $\eta^t$, and iteration times $T$}

Initialize $w_0$ from an arbitrary point in $\cW$

 \For {$t=0$ \textrm{to} $T-1$}{
 Pick $d \sim_u D$ with replacement and compute its gradient $\nabla \ell(w^t;d)$
 
 Let $\Delta^t = \textit{NumericSparse}(\nabla \ell(w^t;d), \alpha, c, \epsilon^{\prime}, \delta^{\prime})$, where $\alpha = \widetilde{O}\Paren{\frac{\sqrt{c}}{\epsilon^{\prime}} }$, $\epsilon^{\prime} = \frac{\epsilon\cdot \ns}{2\sqrt{2T \ln \frac{2}{\delta}}}$ and $\delta^{\prime} = \frac{\delta \ns}{2T}$ \
 
 $w^{t+1} = w^t - \eta^t \Delta^t$\
 }

\KwOut{ $w^{priv} = w^T$}

\caption{Differentially private ERM with sparse gradients }
\label{alg:privatelr}
\end{algorithm}


\begin{theorem}
Algorithm~\ref{alg:privatelr} satisfies $(\eps,\delta)$-DP. 
\end{theorem}

\begin{proof}
We note that in each iteration, when fixing the randomness due to sampling, step 4 itself satisfies $( \epsilon^{\prime}, \delta^{\prime})$-DP, where $\epsilon^{\prime} = \frac{\epsilon\cdot \ns}{2\sqrt{2T \ln \frac{2}{\delta}}}$ and $\delta^{\prime} = \frac{\delta \ns}{2T}$. Then by the following lemma, each iteration ensures $(\frac{\epsilon}{\sqrt{2T \ln \frac{2}{\delta}}}, \frac{\delta}{2T})$-DP. To conclude the proof, we apply the ``strong composition theorem'' (Lemma~\ref{lem:advcomp}) with $\tilde{\delta} = \frac{\delta}{2}$ and $k=T$.
\end{proof}

\begin{theorem}
\label{thm:erm}
Suppose $\forall w,d$, $\normz{\nabla_{\ell(w;d)}} \le c_1$ and $\norminf{\nabla_{\ell(w;d)}}\le c_2$. Additionally, $\forall d$ $\ell(w;d)$ is $L$-smooth in $w$, and $\cL(w^0;D) - \cL(w^*;D) \le D_{\cL}$, where $w^0$ is the starting point, and $w^*$ is the optimal point.
If we set $T= \frac{\ns\eps}{c_1 c_2 }$, then
%then with probability at least $1-\beta$ over the randomness of the algorithm,
\begin{align}
\expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla \cL (w^t)}^2 } = \widetilde{O}\Paren{ \frac{ c_1 c_2 D_{\cL} L }{\ns \eps}+\frac{ c_1 c_2^{1.5} \sqrt{L D_{\ell } }    } {\sqrt{\ns\eps}}  }. \nonumber
\end{align}
%Furthermore, if $\forall d$, $\ell(w;d)$ is convex,
%\begin{align}
%\min \Paren{ \cL(w^t;D) - \cL(w^*;D)  } = \widetilde{O}\Paren{ \frac{ c_1 c_2 D_{\cL} }{\ns \eps}+\frac{ c_1 c_2^{1.5} \sqrt{ D_{\ell } }    } {\sqrt{\ns\eps L}}  }. \nonumber
%\end{align}
Furthermore, we assume $\forall d$ $\ell(w;d)$ is convex in $w$, and $\forall t \in [T]$, $\norm{w^t - w^*} \le D_w$. If we set $T= \frac{\ns\eps}{ \sqrt{c_1} }$, then 
%with probability at least $1-\beta$ over the randomness of the algorithm,

\begin{align}
\expectation{\frac1T \sum_{t=1}^T \Paren{ L(w^t;D) - L(w^*;D) }} &= \widetilde{O}\Paren{ \frac{D_w^2 L \sqrt{c_1}}{\ns\eps} + \frac{D_w c_1^{\frac{3}{4}} c_2 }{\sqrt{\ns\eps}}}.\nonumber
\end{align}

\end{theorem}

\begin{proof}

First by the privacy guarantees of the sparse vector technique (Lemma~\ref{lem:sparsevt}), for each iteration with probability greater than $1-\frac1{n}$,
\begin{align}
&\norminf{\nabla \ell(w;d) - \Delta} \le \frac{2c_2 \sqrt{c_1 T}\Paren{\ln \dims + \ln(4c_1\ns) } \ln \frac{T}{\ns\delta}}{\ns\eps}, \nonumber\\
&\norm{\nabla_{\ell(w;d)} - \Delta} \le \frac{2c_1 c_2 \sqrt{T}\Paren{\ln \dims + \ln(4c_1\ns) } \ln \frac{T}{\ns\delta}}{\ns\eps}. \nonumber
\end{align}
Therefore,
\begin{align}
\expectation{\norm{\nabla_{\ell(w;d)} - \Delta}} &\le \frac{2c_1 c_2 \sqrt{T}\Paren{\ln \dims + \ln(4c_1\ns) } \ln \frac{T}{\ns\delta}}{\ns\eps}+\frac{\sqrt{c_1}c_2}{\ns}\nonumber \\
&\le \frac{4c_1 c_2 \sqrt{T}\Paren{\ln \dims + \ln(4c_1\ns) } \ln \frac{T}{\ns\delta}}{\ns\eps}\nonumber.
\end{align}
Now we apply the following lemma from~\cite{AgarwalSYKM18}.
\begin{lemma}(Corollary 1 in~\cite{AgarwalSYKM18})
Let $\ell$ be $L$-smooth and $D$-Lipschitz. Let $w^0$ satisfy $\cL(w^0;D) - \cL(w^*;D) \le D_{\cL}$. Let $\eta \coloneqq \min \Paren{ \frac1L, \sqrt{2D_\cL} \Paren{\sigma \sqrt{LT}}^{-1} }$, then after $T$ rounds,
$$
\expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla \cL (w^t)}^2} \le \frac{2D_{\cL} L}{T} + \frac{2\sqrt{2} \sigma \sqrt{L D_{\cL}}} {\sqrt{T}}+ DB,
$$
where 
\begin{align}
&\sigma^2 = 2\max_{1\le t \le T} \expectation{\norm{\nabla_{\ell(w;d)} -\nabla \cL(w;D)}^2 } + 2\max_{1\le t \le T} \expectation{\norm{\nabla_{\ell(w;d)} - \Delta}^2}, \text{and} \nonumber\\ 
&B^2= 2\max_{1\le t \le T} \expectation{\norm{\nabla_{\ell(w;d)} - \Delta}^2}. \nonumber
\end{align}
Furthermore, we assume $\forall d$, $\ell(w;d)$ is convex, and $\forall t \in [T]$, $\norm{w^t - w^*} \le D_w$. Let $\eta \coloneqq \min \Paren{ \frac1L, D_w \Paren{\sigma \sqrt{T}}^{-1} }$, then after $T$ rounds.
\begin{align}
\expectation{\frac1T  \sum_{t=1}^T \Paren{ L(w^t;D) - L(w^*;D) }}  \le \frac{D_w^2 L}{T} + \frac{D_w \sigma}{\sqrt{T}}+ 2B D_w\Paren{1 + \frac{D}{\sigma \sqrt{T}}}. \nonumber
\end{align}
\end{lemma}

Note that $\ell$ is $(\sqrt{c_1}c_2)$-Lipschitz, since $\norm{\nabla_{\ell(w;d)}} \le \sqrt{c_1}c_2$. By replacing $D= \sqrt{c_1} c_2$, $B = \frac{c_1 c_2 \sqrt{T}\Paren{\ln \dims + \ln(4c_1\ns) } \ln \frac{T}{\ns\delta}}{\ns\eps}$, and $\sigma^2 = 2B^2 + 2D^2$,
we have 
\begin{align}
\expectation{\frac1{T} \sum_{t=1}^T \norm{\nabla \cL (w^t)}^2 } &\le \frac{2D_{\cL} L }{T}+ \frac{4\sqrt{2} (B+\sqrt{c_1} c_2) \sqrt{L D_{\ell }}} {\sqrt{T}} + \sqrt{c_1}c_2 B  \nonumber
\end{align}
If we take $T = \frac{\ns\eps}{c_1 c_2}$, 
\begin{align}
\frac1{T} \sum_{t=1}^T \norm{\nabla \cL (w^t)}^2  &= O\Paren{ \frac{ c_1 c_2 D_{\cL} L }{\ns \eps}+ \frac{ c_1 c_2^{1.5} \sqrt{L D_{\ell }}} {\sqrt{\ns\eps}} +\frac{ c_1 c_2^{1.5}  \Paren{\ln \dims + \ln(4c_1\ns) } \ln \frac{T}{\ns\delta}  } {\sqrt{\ns\eps}}  }\nonumber\\
& = \widetilde{O}\Paren{ \frac{ c_1 c_2 D_{\cL} L }{\ns \eps}+\frac{ c_1 c_2^{1.5} \sqrt{L D_{\ell } }    } {\sqrt{\ns\eps}}  }. \nonumber
\end{align}
Therefore, we have proved the first part of Theorem~\ref{thm:erm}.

Similarly, for convex loss functions,
\begin{align}
\expectation{\frac1T  \sum_{t=1}^T\Paren{ L(w^t;D) - L(w^*;D) }  }\le \frac{D_w^2 L}{T} + \frac{D_w (B+\sqrt{c_1} c_2 )}{\sqrt{T}}+ 2B D_w\Paren{1 + \frac{\sqrt{c_1}c_2}{(B+\sqrt{c_1}c_2)\sqrt{T}}}. \nonumber
\end{align}
If we take $T = \frac{\ns\eps}{\sqrt{c_1}}$,
\begin{align}
\frac1T  \expectation{\sum_{t=1}^T \Paren{ L(w^t;D) - L(w^*;D) }}  &= O\Paren{  \frac{D_w^2 L \sqrt{c_1}}{\ns\eps} + \frac{D_w c_1^{\frac{3}{4}} c_2 }{\sqrt{\ns\eps}}+ \frac{2D_w c_1^{\frac{3}{4}} c_2  \Paren{\ln \dims + \ln(4c_1\ns) } \ln \frac{T}{\ns\delta}}{\sqrt{\ns\eps}}  } \nonumber\\
&= \widetilde{O}\Paren{ \frac{D_w^2 L \sqrt{c_1}}{\ns\eps} + \frac{D_w c_1^{\frac{3}{4}} c_2 }{\sqrt{\ns\eps}}}.\nonumber
\end{align}

%For the second part, we need the following property of convex smooth functions:
%
%\begin{lemma}
%\label{lem: property_smooth_convex}
%Let $\ell$ be a convex and $L$-smooth function on $\mathbb{R}^{\dims}$, 
%$$f(y) - f(x) - \nabla f (x)^ T (y-x) \ge \frac1{2L} \norm{\nabla f(y) - \nabla f(x)}^2 , ~~~ \forall x,y \in \mathbb{R}^{\dims}.$$\end{lemma}
%
%Let $w^{t^\prime} = \arg\min {\ell(w^t;D)}$, by Lemma~\ref{lem: property_smooth_convex},
%
%
%\begin{align}
%\min \Paren{ \cL(w^t;D) - \cL(w^*;D)  } = \widetilde{O}\Paren{ \frac{ c_1 c_2 D_{\cL} }{\ns \eps}+\frac{ c_1 c_2^{1.5} \sqrt{ D_{\ell } }    } {\sqrt{\ns\eps L}}  }. \nonumber
%\end{align}

\end{proof}








%Now if we further assume the data set $D$ is drawn i.i.d.\ from some underlying distribution $P$, the following lemma from learning theory relates the true risk and the empirical risk, which shall be heavily used in the following sections.
%
%\begin{theorem}
%\label{thm:generalization_error}
%If we consider the same problem setting and assumptions as in Corollary~\ref{cor:EmpiricalError}, and we further assume that the training data set $D$ is drawn i.i.d.\ from some unknown distribution $P$, then with probability at least $1-\beta$ over the randomness of the algorithm and the training data set,
%$$ \expectationf{\ell(w^{priv};(X,Y))}{(X,Y)\sim P} - \expectationf{\ell(w^*;(X,Y))}{(X,Y)\sim P}  = O\Paren{ \frac{\lambda^{\frac{4}{3}}\log(\frac{ \ns\dims}{\beta}) } {(\ns \sqrt{\rho})^{\frac{2}{3}}} + \frac{\lambda \log\Paren{\frac1{\beta}}}{\sqrt{n}} },$$
%where $w^* = \arg\min_{w\in C}\expectationf{\ell(w;(X,Y))}{(X,Y)\sim P} $.
%\end{theorem}
%
%\begin{proof}
% By triangle inequality,
%\begin{align*}
%&~\expectationf{\ell(w^{priv};(X,Y))}{(X,Y)\sim P} - \expectationf{\ell(w^*;(X,Y))}{(X,Y)\sim P} \nonumber\\
%\le& \absv{ \expectationf{\ell(w^{priv};(X,Y))}{(X,Y)\sim P} - \frac1{\ns} \sum_{m=1}^{\ns} \ell(w^{priv};d^m) } + \absv{  \frac1{\ns}\sum_{m=1}^{\ns} \ell(w^{priv};d^m) - \frac1{\ns}\sum_{m=1}^{\ns} \ell(w^{erm};d^m) } \nonumber\\
%+& \Paren{  \frac1{\ns}\sum_{m=1}^{\ns} \ell(w^{erm};d^m) - \frac1{\ns}\sum_{m=1}^{\ns} \ell(w^*;d^m) } + \absv{ \expectationf{\ell(w^{*};(X,Y))}{(X,Y)\sim P} - \frac1{\ns}\sum_{m=1}^{\ns} \ell(w^{*};d^m) } \nonumber
%\end{align*}
%
%Now we need to bound each term. We firstly bound the first and last term simultaneously. By the generalization error bound (Lemma 7 from~\cite{WuSD19}), they are bounded by $O\Paren{ \frac{\lambda \log\Paren{\frac1{\beta}}}{\sqrt{n}}}$ simultaneously, with probability greater than $1 - \frac{2}{3}\beta$. Then we turn to the second term, by Corollary~\ref{cor:EmpiricalError}, with probability greater than $1 - \frac{1}{3}\beta $, it is bounded by $ O\Paren{ \frac{\lambda^{\frac{4}{3}}\log(\frac{ \ns\dims}{\beta}) } {(\ns \sqrt{\rho})^{\frac{2}{3}}}}$. Finally we bound the third term. According to the definition of $w^{erm}$, the third term should be smaller than 0.
%Therefore, by union bound, $ \expectationf{\ell(w^{priv};(X,Y))}{(X,Y)\sim P} - \expectationf{\ell(w^*;(X,Y))}{(X,Y)\sim P}  = O\Paren{ \frac{\lambda^{\frac{4}{3}}\log(\frac{ \ns\dims}{\beta}) } {(\ns \sqrt{\rho})^{\frac{2}{3}}} + \frac{\lambda \log\Paren{\frac1{\beta}}}{\sqrt{n}} }$, with probability greater than $1-\beta$.
%\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

